Semi-supervised Learning with Network Embedding on Ambient RF Signals for Geofencing Services

In applications such as elderly care, dementia anti-wandering and pandemic control, it is important to ensure that people are within a predefined area for their safety and well-being. We propose GEM, a practical, semi-supervised Geofencing system with network EMbedding, which is based only on ambient radio frequency (RF) signals. GEM models measured RF signal records as a weighted bipartite graph. With access points on one side and signal records on the other, it is able to precisely capture the relationships between signal records. GEM then learns node embeddings from the graph via a novel bipartite network embedding algorithm called BiSAGE, based on a Bipartite graph neural network with a novel bi-level SAmple and aggreGatE mechanism and non-uniform neighborhood sampling. Using the learned embeddings, GEM finally builds a one-class classification model via an enhanced histogram-based algorithm for in-out detection, i.e., to detect whether the user is inside the area or not. This model also keeps on improving with newly collected signal records. We demonstrate through extensive experiments in diverse environments that GEM shows state-of-the-art performance with up to 34% improvement in F-score. BiSAGE in GEM leads to a 54% improvement in F-score, as compared to the one without BiSAGE.

==> revision/system_overview.tex <==


%Users collect training signals inside the house during initial walks, then they are free to move. \n{} builds a bipartite graph with training data to generate embeddings for boundary discovery. The boundary is then used to detect whether a testing sample is in premises or not (i.e., absconder alert). Highly confident in-premises signals are used to update the boundary.


%\subsection{Design Considerations}
%\label{subsec:d_challenge}
%
%%A practical geofencing system needs to work even when the AP environment varies significantly. Furthermore, it should be easy to use and requires minimum intervention from users. We consider the following technical challenges in designing \n{}.
%
%We make the following considerations in designing \n{} so that it can be easy to use and requires minimal intervention from users while being robust to the environmental factors.
%
%\begin{itemize}[itemsep=2pt,leftmargin=1.5em]
%    \item \emph{Geofencing without maps and location labels.} It is not practical to ask users to obtain their house floorplans nor feasible to `label' exact locations when measuring RSS values from ambient APs, thereby making the localization-based techniques~\cite{abbas2019wideep} inappropriate for geofencing. \n{} is designed to build a one-class classification model for in-out detection based only on the RSS values \emph{without} any exact location labels.
%
%        %To address this issue, \n{} exploits one-class classification techniques that require users to report signals from inside the house without any exact location label.
%
%    \item \emph{No extra hardware.} Using extra hardware~\cite{geofencing09} for geofencing is often labor-intensive and costly. \n{} merely uses ambient RF signal records, which are easily collected on almost all smartphones and IoT wearables, such that users simply run an application on their devices.
%
%    \item \emph{Initial training in a short time.} For easy adoption of \n{}, it is desirable to minimize the intervention from users in the initial data collection process. For \n{}, each user with an IoT device is only asked to move along the inner perimeter of the geofencing area for a just few minutes initially. The user can just stay as usual afterwards.
%
%    \item \emph{Robustness to dynamic RF environments.} To make \n{} highly accurate for in-out detection, the detection model should be not only robust to spatial and temporal changes in the recorded RSS values but also capture their dynamics. Note that sensed APs and recorded RSS values can vary spatially and temporally. The number of detected APs can even easily change with a slight movement. In addition, the (initial) model should be based only on a limited number of RF signal records. \n{} builds an accurate and robust model based on the weighted bipartite graph modeling, \bisage{}, and the histogram-based detection algorithm. \n{} is also able to further enhance the model over time.
%
%\end{itemize}

%We find it challenging to capture spatial and temporal RSS distribution during the geofencing period, especially when we have only a limited time for measurement in the training phase. Also, with a slight movement, the number of detected APs may easily change in the same place, such as corners. Hence, how to capture such severe RF signal dynamics becomes a big challenge.



% {\color{blue} move to Sec. 2.2, minimize information loss; small number of testing samples; General flow -> problem -> module design.}
% \textbf{Scalability based on bipartite graph modeling of signals.} The new perspective of modeling RF signals with the bipartite graph is inspired by the inherent structure of RF signal collection, where observations and APs are connected with RSS measurements.

% \begin{itemize}
%     \item \emph{Flexibility in model extension.} RSS distribution is difficult to capture, especially when we only have limited measurement time. The number of APs detected may easily change at the same place, such as corners. Our bipartite graph modeling in \n{} for APs and observations (\S\ref{subsec:bipartite}) enables easy addition and removal of nodes and edges, ensuring that RSS collected can be well modeled.

%     \item \emph{Learning with a large number of testing samples.} As we have limited initial training time, there may be only peripheral signals collected, as such, the initially learned signal boundary is not accurate. Since it is not favorable for confinees to receive false alarms, \n{} seeks to improve the detection performance efficiently over time by leveraging a significantly large number of testing samples. Our online learning mechanism is two-folded. We first update the bipartite graph (\S\ref{subsec:graph_update}) and embeddings in an unsupervised manner (\S\ref{subsec:nl_update}), and then leverage highly confident predicted inliers (\S\ref{subsec:b_update}) to update the signal boundary. Over a short geofencing period, such as pandemic quarantine, the number of nodes in the network can quickly grow to tens of thousands. With network embedding, we can efficiently cope with this complexity and provide reliable geofencing service.
% \end{itemize}


%\subsection{System Overview}
%\label{subsec:sys_overview}

We first provide a system overview of \n{}, as shown in Figure~\ref{fig:sys_overview}, before we go into the details. Within a geofencing area, a user wearing an IoT device is asked to move roughly along the perimeter \emph{inside} the area to collect RF signal records from ambient APs for a few minutes. The user is then free to move around and just lives as usual. On the other hand, the collected `in-premises' records are used to train a one-class classification model, and \n{} is ready to use. \n{} continues to update the model over time with new RF signal records that are collected from the IoT device on a regular basis while performing in-out detection.

%, which is to detect whether the user is inside the area or outside

%, inspired by the inherent structure of RF signal measurements where each one consists of sensed APs and their corresponding RSS values

%Once the initial set of RF signal records (samples) are collected,

The one-class classification model is built as follows. We first model RF signal records and their relationships through a weighted bipartite graph (Section~\ref{subsec:bipartite}). The bipartite graph is then processed with our novel network embedding algorithm \bisage{} (Section~\ref{subsec:bisage}) to learn node embeddings in an unsupervised manner. Finally, the learned embeddings are used to train an in-out detection model via our enhanced histogram-based in-out detection algorithm (Section~\ref{subsec:boundary_training}). Our initial detection model in \n{} may not be accurate enough due to the limited amount of training data. Thus, while \n{} records RSS values from ambient APs on a regular basis for in-out detection, they are also leveraged to further enhance the model. Specifically, when a new RF signal record becomes available, it is added into the bipartite graph and its embedding is obtained through the learned \bisage{} model (Section~\ref{subsec:graph_update}). The embedding is then fed into the detection model for in-out detection. While doing so, if predicted to be a highly confident in-premises sample, it is used to update our detection model to improve its performance (Section~\ref{subsec:b_update}). This self-enhancement continues over time.


%The initially learned signal boundary may not be accurate enough due to limited initial training time. Since it is not favorable for confinees to receive false alarms, \n{} seeks to improve the detection performance efficiently over time by leveraging a large number of testing samples\footnote{We call samples collected continuously after the initial training as testing samples.} collected after the initial training. In particular, this process is integrated with the online inference and update process, which consists of two steps: we first incorporate measurement samples into the bipartite graph and then generate node embeddings with the trained aggregator (Section~\ref{subsec:graph_update}). We then leverage highly confident predicted in-premises signals (Section~\ref{subsec:b_update}) to update the signal boundary so that the system performance can be improved over time.



% \jinsung{It would be better to explain a key idea on how to classify between inlier and outlier before diving into the detailed algorithm.
% Actually, I found Figure 2 shows how-to, but there is no corresponding text in this subsection.}

% These in-boundary RF signals are first used to build a bipartite graph (\S\ref{subsec:bipartite}).

%  With more incoming testing signals, the bipartite graph incorporates them to generate new latent representations (\S\ref{subsec:graph_update}). Meanwhile, old representations that are mostly affected by these newly added nodes are updated (\S\ref{subsec:nl_update}). The representation update process is unsupervised. Afterwards, \n{} predicts in/out labels for these testing representations with learned boundary. If outliers are detected, an alarm will be triggered. Otherwise, each inlier is associated with a prediction score. Those inliers with prediction scores lower than a threshold are then used to update the signal boundary (\S\ref{subsec:b_update}). This way, the classification model improves over time.




% We overview \n{} in Fig.~\ref{fig:sys_overview}. During {\em offline training}, the confinee, attached with an IoT device, collects in-premise RF signals for some, say 10, minutes. The collected RF signals are inliers, and are used for offline training of the one-class classification model. These in-boundary RF signals are first used to build a bipartite graph for network training. The bipartite graph is processed with network embedding to learn corresponding latent representation for each node in an unsupervised manner.\footnote{We use latent representation and embedding interchangeably.} The learnt representations are then processed with one-class classification model for initial boundary discovery.

% After initial walks, the confinee is free to move, and our system enters into  {\em online update} phase. With incoming testing signals, the bipartite graph is first expanded to incorporate these new signals in network update. Latent representations are then generated for newly added nodes in the graph. Meanwhile, old representations that are mostly affected by these newly added nodes are updated. The network update is an unsupervised process. Afterwards, \n{} predicts in/out labels for the new nodes, and attach with each new node a confidence score. Those inliers with high confidence scores are then used to update the signal boundary. This way, the classification model improves over time. With network embedding, the whole updating process is highly efficient and scalable for geofencing decision. 
